Grover's oracle for the Shortest Vector Problem and its application in hybrid classical-quantum solvers

Finding the shortest vector in a lattice is a problem that is believed to be hard both for classical and quantum computers. Many major post-quantum secure cryptosystems base their security on the hardness of the Shortest Vector Problem (SVP). Finding the best classical, quantum or hybrid classical-quantum algorithms for SVP is necessary to select cryptosystem parameters that offer sufficient level of security. Grover's search quantum algorithm provides a generic quadratic speed-up, given access to an oracle implementing some function which describes when a solution is found. In this paper we provide concrete implementation of such an oracle for the SVP. We define the circuit, and evaluate costs in terms of number of qubits, number of gates, depth and T-quantum cost. We then analyze how to combine Grover's quantum search for small SVP instances with state-of-the-art classical solvers that use well known algorithms, such as the BKZ, where the former is used as a subroutine. This could enable solving larger instances of SVP with higher probability than classical state-of-the-art records, but still very far from posing any threat to cryptosystems being considered for standardization. Depending on the technology available, there is a spectrum of trade-offs in creating this combination.

==> gates_implementation.tex <==

\subsection{Implementation of a quantum full-adder circuit}
There exist two kinds of carry propagate adders: 1. \textit{Ripple-carry adders} which sequentially chain full-adders (adders with carry input and output) 2. \textit{Carry-lookahead adders} which perform a more efficient addition in terms of depth by dividing the addition into blocks. In general, ripple-carry adders have a lower cost th the expense of their depth and carry-lookahead adders tradeoff lower depth for the higher cost. Moreover, there exist different quantum circuit implementations of each of them and the choice depends not only on preference on the resource trade-off, but also on the gate set available in an architecture considered. We list the state-of-the-art implementations in Table \ref{fig:table_adders}. In terms of optimal trade-off of resources and depth, \cite{li2020efficient, Thapliyal2013} seem in general to be better suited in for ripple-carrry adders and \cite{Thapliyal2013ProgressIR} for carry-lookahead adders. 

\begin{table}[h]\label{fig:table_adders}
	\begin{tabular}{lllll}
		{\ul }              & Quantum Cost{\ul }&\# of Ancillas {\ul} & Delay $\Delta$ {\ul } & Type {\ul } \\ \cline{2-5} 
		\multicolumn{1}{l|}{\cite{li2020efficient}} &      $13N-10$ &    $0$    & $10N-4$       &   Ripple-Carry     \\
		\multicolumn{1}{l|}{\cite{Thapliyal2013}} &   $13N-8$     &    $0$    & $11N-4$       & Ripple-Carry     \\
		\multicolumn{1}{l|}{\cite{Thapliyal2013ProgressIR}} &    $26N-15W(N)-15\log(N-4)$    &    $5N/4$   &   $\log N + \log\frac{N}{3}+2$      &   Carry-Lookahead    
	\end{tabular}
\end{table}
Another approach is the use of Quantum Fourier Transform for performing the addition as firstly proposed by \cite{qftAddition}.

\subsection{Implementation of a quantum full subtractor circuit}
\begin{table}[h]\label{fig:table_subtractors}
	\begin{tabular}{llll}
		{\ul }  & Quantum Cost{\ul }&\# of Ancillas {\ul} & Delay $\Delta$ {\ul } \\ \cline{2-4} 
		\multicolumn{1}{l|}{\cite{adder} \#1} &      $6N-3$ &    $0$    & $6N-3$        \\
		\multicolumn{1}{l|}{\cite{adder} \#2} &   $16N-8$     &    $0$    & $13N-9$     \\
		\multicolumn{1}{l|}{\cite{adder} \#3} &    $16N-6$    &    $1$   &   $9N+2$   
	\end{tabular}
\end{table}


\subsection{Implementation of a quantum full adder-subtractor circuit}
\cite{adder} proposes three approaches (the second approach is omitted due to being non-optimal) to construct reversible full adders/subtractors controlled by a single control qubit. The Approach 1 is to use a ripple-carry adder composed of full adders proposed by \cite{Maslov2006QuantumCS}. The control qubit, if switched on, changes a sign of the second input $b$ by performing two's complement complement using \textit{XOR} operations and adding 1. The second approach substitutes the full adder by the one in \cite{subtractor}. Compared to the one used in the Approach 1, it requires no additional ancillary qubit with the price of an increased delay. 
\begin{table}[h]\label{fig:table_adders}
	\begin{tabular}{lllll}
		{\ul }              & Quantum Cost{\ul }&\# of Ancillas {\ul} & Delay $\Delta$ {\ul }  \\
		 \cline{2-5} 
		\multicolumn{1}{l|}{Approach 1} &      $7N+1$ &    $N+1$    & $4N+1$    \\
		\multicolumn{1}{l|}{Approach 3} &   $16N-6$     &    $0$    & $9N+2$ 
	\end{tabular}
\end{table}
\input{adder_subtractor.tex}
\input{adder_subtractor_approach3.tex}
\subsection{Implementation of a multiplier}
There exist two known approaches to implementing quantum circuits performing multiplication. The first one, also used in Qiskit \cite{Qiskit} as a default choice, uses a sequence of adders whose number is determined by an ensemble of control bits which carry a binary representation if a multiplicand and so they essentially control number of adders being used. As argued by \cite{quoc_2004}, a naive implementation of a multiplier as a sequence of adders is inefficient for qubit count due to requirements of ancillary qubits for implementation of carry. Instead, the authors propose use of Quantum Fourier Transform

\begin{figure}[h!]
		\label{circ_diagram_multiplier}
	\input{multiplier.tex} 
	\caption{Implementation of multiplier as an unfolded sum}
\end{figure}


\subsection{Implementation of a square circuit}
\cite{circDesignForTrans} proposes that the square circuit can be obtained by reversing the circuit for square root operation, and
the square root circuit can be designed based on the non-restoring method.  Requires $n$ ancillas, but seems as a better choice than repeating parts of the circuit in parallel twice (that would introduce more qubits). Such an example is in \cite{qFastPoissonSolver} which proposes a circuit for a square root and its inverse. Also, take a look at \cite{squares}, they claim 63\% constant improvement for ancillas and gate count.

\subsection{Implementation of the final comparator}
The final part of the circuit compares the output vector with the constant multiple of a Gaussian heuristics specified apriori. The usual procedure is to perform a subtraction as the output is then saved in the carry qubit. TODO: study if sth better can be done, although this seems to be pretty good as it scales linearly with $n$

\subsection{Handling of integer signs in binary representations}
Since enumeration coefficients are allowed to be both positive and negative, our quantum circuit needs to keep track of signs of the integer representations (\textcolor{violet}{violet}) color in the Figure \ref{circ_diagram}. Note, that each row of $B$ can be multiplied by $-1$ in a way that $B_{0\cdot}\geq 0$ which saves us resources as we do not need to handle this case. TODO: explain in detail how the sign is handled

==> list_of_commented_out.tex <==
\petros{TODO: list of convention/notation choices: T-gate (change t-gate); -ize (change the -ise); check corss-references especially since we changed section}

\petros{We need to include here: (a) other works on Grover oracle implementations (non-SVP), (b) works on quantum SVP (FT and NISQ), (c) recent works on Grover and SVP (perhaps stating ``independent'' for things that happen in parallel to us)}

From preliminaries:
\milos{
\begin{definition}[Gram-Schmidt decomposition]
	\textcolor{red}{to do}
\end{definition}
}\milos{
\begin{definition}[Gramian of the lattice]
	Let $\bl$ be an $m$-dimensional basis whose rows are the basis vectors of $\mathcal{L}$. Then $G(\mathcal{L}):=BB^T$ is called a Gram (or Gramian) matrix of the basis $\bl$.
\end{definition}}
\milos{
\begin{definition}[Volume of the lattice]
	The volume of the lattice $\mathcal{L}$ is defined as
	$$
	\text{vol}(\mathcal{L})=|\det\bl|
	$$ and as argued by \cite{Nguyen2010}, it is independent of the underlying lattice basis.
\end{definition}}
\milos{
\begin{proposition}There are multiple ways to express the volume of the lattice:
	$$\text{vol}(\mathcal{L})=|\det\bl|=\sqrt{\det G(\mathcal{L})}=\prod_i||b_i^*||$$
\end{proposition}}
\milos{
\begin{proof}
	\cite{Micciancio_2010,Nguyen2010} where $B^*$ is Gram-Schmidt orthogonalization of $B$. 
\end{proof}
}
\milos{
\begin{definition}[Hermite's constant]
	Hermite's constant $\gamma_n$ is defined as
	$$
	\gamma_n:=\sup_{\mathcal{L}\in\mathbb{L}_n}\left\{\frac{\lambda_1(\mathcal{L})^2}{\text{vol}(\mathcal{L})^{2/n}}\right\}
	$$ where the supremum is taken over set of all possible $n$-rank lattices.
\end{definition}
}\milos{
\begin{proof}
	\cite{Nguyen2010}
\end{proof}}
\milos{
\begin{proposition}[Number of lattice vectors points inside a measurable body]
Let $\mathcal{B}\subset\mathbb{R}^n$ be a measurable body
$$
|\mathcal{L}\cap\mathcal{B}|\approx\frac{\text{Vol}(\mathcal{B})}{\text{Vol}(\mathcal{L})}
$$
\end{proposition}
}
\milos{
\begin{definition}[Minkowski's Theorem]\cite{Minkowski1953}
    Let $S$ be a centrally-symmetric convex set of volume greater than $2^n\det(\mathcal{L})$. Then $S$ contains a non-zero point in $\mathcal{L}$.
\end{definition}
}
\milos{\begin{corollary}[Corollary of Minkowski's Theorem]
    \cite{Kelner2009} $$\lambda_1(\mathcal{L})\leq\sqrt{n}(\det(\mathcal{L}))^{1/n}$$
\end{corollary}}




\milos{TODO: Mention that this work uses the same figures of merit: \cite{aesResourceEstimation} implements Grover's oracles different key sizes of Advanced Encryption Standard (AES). They decompose the circuits into Clifford+T set and argue about qubit and depth requirements.}

\milos{being a crude overapproximation}

\petros{[TODO: if we are to include the overall cost of Grover's algorithm here we should remove section 6 and merge any content needed in this section.]}

%\petros{[First write the costs for single Grover iteration; Then multiply to get the Grover's algorithm]}

\petros{[last sentence is very informal and not quite accurate (VQAs would also suffer for similar time complexity given that the probability of success of a single run would be exponentially small). also the point is that you wouldn't brute force it (classically or quantumly) but you could use it for solving smaller instances that hepls as in the next section.]}

==> table_grover_counts.tex <==
\begin{tabular}{l|rrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45 & 46 & 47 & 48 & 49 & 50 & 51 & 52 & 53 & 54 & 55 & 56 & 57 & 58 & 59 & 60 & 61 & 62 & 63 & 64 & 65 & 66 & 67 & 68 & 69 & 70 & 71 & 72 & 73 & 74 & 75 & 76 & 77 & 78 & 79 & 80 & 81 & 82 & 83 & 84 & 85 & 86 & 87 & 88 & 89 & 90 & 91 & 92 & 93 & 94 & 95 & 96 & 97 & 98 & 99 & 100\\
\hline
num\_iters & 2 & 3 & 3 & 4 & 4 & 4 & 4 & 5 & 5 & 5 & 5 & 5 & 6 & 6 & 6 & 6 & 6 & 6 & 7 & 7 & 7 & 7 & 7 & 7 & 7 & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 8 & 9 & 9 & 9 & 9 & 9 & 9 & 9 & 9 & 9 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 10 & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 11 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 12 & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 13 & 14 & 14 & 14 & 14 & 14 & 14 & 14 & 14 & 14 \\
gate\_count & 7554 & 20904 & 32904 & 63716 & 87324 & 114812 & 144972 & 224145 & 271765 & 324670 & 380070 & 441125 & 608298 & 693966 & 781686 & 876678 & 977382 & 1085304 & 1393308 & 1529479 & 1672405 & 1824221 & 1976121 & 2137667 & 2305961 & 2838544 & 3040464 & 3254056 & 3475384 & 3708232 & 3938472 & 4181032 & 4431368 & 5280624 & 5571504 & 5876973 & 6191217 & 6519951 & 6842691 & 7180749 & 7527609 & 7889742 & 9160380 & 9572250 & 9993950 & 10433330 & 10862730 & 11310810 & 11768770 & 12245240 & 12710040 & 13194330 & 13688550 & 15622321 & 16172541 & 16745091 & 17328597 & 17934334 & 18523494 & 19135875 & 19759245 & 20405803 & 21033903 & 21686115 & 24381132 & 25130976 & 25858656 & 26613612 & 27380652 & 28175028 & 28945188 & 29743596 & 30554124 & 31393032 & 32205672 & 33047532 & 36726677 & 37683737 & 38610117 & 39569205 & 40541501 & 41546804 & 42519204 & 43525365 & 44544851 & 45598319 & 46616739 & 47670025 & 48736623 & 49838282 & 54818316 & 56003318 & 57202698 & 58441054 & 59636934 & 60872630 & 62122774 & 63413056 & 64658496 \\
depth & 1226 & 2316 & 2883 & 4048 & 4596 & 5264 & 6304 & 7715 & 8385 & 9280 & 10955 & 10370 & 13254 & 14328 & 16836 & 15630 & 16422 & 17496 & 23947 & 21952 & 22883 & 24192 & 28252 & 25669 & 26579 & 31888 & 37208 & 33584 & 34600 & 36128 & 42128 & 37832 & 38824 & 45396 & 52929 & 47340 & 48429 & 50148 & 58464 & 52119 & 53181 & 54972 & 71110 & 63220 & 64410 & 66400 & 77260 & 68530 & 69690 & 71680 & 83410 & 73840 & 74970 & 84678 & 98516 & 87065 & 88275 & 90486 & 105281 & 92906 & 94083 & 96316 & 112046 & 98747 & 108972 & 111408 & 129612 & 114096 & 115308 & 117744 & 136992 & 120468 & 121644 & 124080 & 144372 & 126840 & 138645 & 141284 & 164398 & 144313 & 145509 & 148148 & 172393 & 151216 & 152425 & 155116 & 180388 & 158119 & 159289 & 162006 & 202874 & 177716 & 178934 & 181888 & 211484 & 185150 & 186326 & 189280 & 220094 \\
tdepth & 404 & 741 & 936 & 1760 & 1492 & 1676 & 1984 & 3475 & 2720 & 2955 & 3390 & 4750 & 4290 & 4554 & 5088 & 7230 & 5316 & 5562 & 7112 & 10220 & 7399 & 7693 & 8372 & 12005 & 8596 & 10136 & 10928 & 15760 & 11192 & 11480 & 12288 & 17800 & 12560 & 14427 & 15336 & 22320 & 15669 & 15939 & 16848 & 24615 & 17208 & 17487 & 20500 & 29900 & 20830 & 21110 & 22200 & 32450 & 22540 & 22790 & 23900 & 35000 & 24250 & 26917 & 28138 & 41305 & 28556 & 28765 & 29986 & 44110 & 30437 & 30613 & 31856 & 46915 & 35256 & 35412 & 36768 & 54240 & 37308 & 37428 & 38784 & 57300 & 39360 & 39444 & 40800 & 60360 & 44863 & 44915 & 46384 & 68705 & 47086 & 47099 & 48568 & 72020 & 49309 & 49335 & 50856 & 75335 & 51532 & 51519 & 57148 & 84700 & 57890 & 57834 & 59528 & 88270 & 60284 & 60186 & 61880 \\
\end{tabular}

==> table_oracle_counts.tex <==
\begin{tabular}{l|rrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45 & 46 & 47 & 48 & 49 & 50 & 51 & 52 & 53 & 54 & 55 & 56 & 57 & 58 & 59 & 60 & 61 & 62 & 63 & 64 & 65 & 66 & 67 & 68 & 69 & 70 & 71 & 72 & 73 & 74 & 75 & 76 & 77 & 78 & 79 & 80 & 81 & 82 & 83 & 84 & 85 & 86 & 87 & 88 & 89 & 90 & 91 & 92 & 93 & 94 & 95 & 96 & 97 & 98 & 99 & 100\\
\hline
gate\_count & 3763 & 6910 & 10963 & 15922 & 21787 & 28558 & 36235 & 44818 & 54307 & 64702 & 76003 & 88210 & 101323 & 115342 & 130267 & 146098 & 162835 & 180478 & 199027 & 218482 & 238843 & 260110 & 282283 & 305362 & 329347 & 354238 & 380035 & 406738 & 434347 & 462862 & 492283 & 522610 & 553843 & 585982 & 619027 & 652978 & 687835 & 723598 & 760267 & 797842 & 836323 & 875710 & 916003 & 957202 & 999307 & 1042318 & 1086235 & 1131058 & 1176787 & 1223422 & 1270963 & 1319410 & 1368763 & 1419022 & 1470187 & 1522258 & 1575235 & 1629118 & 1683907 & 1739602 & 1796203 & 1853710 & 1912123 & 1971442 & 2031667 & 2092798 & 2154835 & 2217778 & 2281627 & 2346382 & 2412043 & 2478610 & 2546083 & 2614462 & 2683747 & 2753938 & 2825035 & 2897038 & 2969947 & 3043762 & 3118483 & 3194110 & 3270643 & 3348082 & 3426427 & 3505678 & 3585835 & 3666898 & 3748867 & 3831742 & 3915523 & 4000210 & 4085803 & 4172302 & 4259707 & 4348018 & 4437235 & 4527358 & 4618387 \\
depth & 610 & 742 & 874 & 1006 & 1138 & 1270 & 1402 & 1534 & 1666 & 1798 & 1930 & 2062 & 2194 & 2326 & 2458 & 2590 & 2722 & 2854 & 2986 & 3118 & 3250 & 3382 & 3514 & 3646 & 3778 & 3910 & 4042 & 4174 & 4306 & 4438 & 4570 & 4702 & 4834 & 4966 & 5098 & 5230 & 5362 & 5494 & 5626 & 5758 & 5890 & 6022 & 6154 & 6286 & 6418 & 6550 & 6682 & 6814 & 6946 & 7078 & 7210 & 7342 & 7474 & 7606 & 7738 & 7870 & 8002 & 8134 & 8266 & 8398 & 8530 & 8662 & 8794 & 8926 & 9058 & 9190 & 9322 & 9454 & 9586 & 9718 & 9850 & 9982 & 10114 & 10246 & 10378 & 10510 & 10642 & 10774 & 10906 & 11038 & 11170 & 11302 & 11434 & 11566 & 11698 & 11830 & 11962 & 12094 & 12226 & 12358 & 12490 & 12622 & 12754 & 12886 & 13018 & 13150 & 13282 & 13414 & 13546 \\
tdepth & 198 & 240 & 282 & 324 & 366 & 408 & 450 & 492 & 534 & 576 & 618 & 660 & 702 & 744 & 786 & 828 & 870 & 912 & 954 & 996 & 1038 & 1080 & 1122 & 1164 & 1206 & 1248 & 1290 & 1332 & 1374 & 1416 & 1458 & 1500 & 1542 & 1584 & 1626 & 1668 & 1710 & 1752 & 1794 & 1836 & 1878 & 1920 & 1962 & 2004 & 2046 & 2088 & 2130 & 2172 & 2214 & 2256 & 2298 & 2340 & 2382 & 2424 & 2466 & 2508 & 2550 & 2592 & 2634 & 2676 & 2718 & 2760 & 2802 & 2844 & 2886 & 2928 & 2970 & 3012 & 3054 & 3096 & 3138 & 3180 & 3222 & 3264 & 3306 & 3348 & 3390 & 3432 & 3474 & 3516 & 3558 & 3600 & 3642 & 3684 & 3726 & 3768 & 3810 & 3852 & 3894 & 3936 & 3978 & 4020 & 4062 & 4104 & 4146 & 4188 & 4230 & 4272 & 4314 \\
\end{tabular}

